Energy-aware Load Balancing Policies for the Cloud Ecosystem

The energy consumption of computer and communication systems does not scale linearly with the workload. A system uses a significant amount of energy even when idle or lightly loaded. A widely reported solution to resource management in large data centers is to concentrate the load on a subset of servers and, whenever possible, switch the rest of the servers to one of the possible sleep states. We propose a reformulation of the traditional concept of load balancing aiming to optimize the energy consumption of a large-scale system: {\it distribute the workload evenly to the smallest set of servers operating at an optimal energy level, while observing QoS constraints, such as the response time.} Our model applies to clustered systems; the model also requires that the demand for system resources to increase at a bounded rate in each reallocation interval. In this paper we report the VM migration costs for application scaling.

==> CloudEnergyConsumption.tex <==
%*********************************************************************************
\section{Energy Consumption of Large-scale Data Centers}
\label{CloudEnergyConsumption}
\medskip
%*********************************************************************************

The energy used for IT activities represents a significant and continually increasing component of the total energy used by a nation; its ecological impact is of serious concern. Thus, it is no surprise that energy optimization is an important dimension of the cloud resource management policies.

{\bf Cloud computing.} Cloud computing has the potential to reduce the energy consumption for computing and data storing thus, shrink the carbon footprint for IT-related activities. This potential is far from being realized by existing cloud infrastructures.

The rapid expansion of the cloud computing community helps us realize the full impact of cloud computing on the energy consumption in the US and the world. The number of Cloud Service Providers (CSPs), the spectrum of services offered by the CSPs, and the number of cloud users have increased dramatically during the last few years. For example, in 2007 the EC2 (Elastic Cloud Computing) was the first service provided by AWS (Amazon Web Services); five years later, in 2012, AWS was used by businesses in 200 countries. Amazon's S3 (Simple Storage Service) has surpassed two trillion objects and routinely runs more than 1.1 million peak requests per second; the Elastic MapReduce has launched 5.5 million clusters since the start of the service in May 2010 (ZDNet 2013). A recent posting on ZDNet reveals that in January 2012 EC2 was made up of 454,600 servers. When one adds the number of servers supporting other AWS services, then the total number of Amazon systems dedicated to cloud computing is much larger. An unofficial estimation puts the number of servers used by Google in January 2012 close to 1.8 million; this number was expected to be close to 2.4 million by the early 2013.

The costs for maintaining the cloud computing infrastructure are significant. A large fraction of these costs are for data center housing and cooling and for powering the computational and storage servers and the interconnection networks. Indeed, it was predicted that by 2012 up to $40\% $of the budget of IT enterprise infrastructure will be spent on energy. The energy costs are different in different countries and in different regions of the same country. While most of the power for large data centers, including cloud computing centers, comes from power stations burning fossil fuels such as coal and gas, in recent years the contribution of solar, wind, geothermal and other renewable energy sources has steadily increased.

The infrastructure supporting IT industry and cloud computing in particular has become a major consumer of electric power. The power consumption of large-scale data centers and their costs for energy and for cooling are significant and are expected to increase in the future. In $2006$, the $6\,000$ data centers in the U.S. reportedly consumed $61 \times 10^{9}$ KWh of energy, $1.5\%$ of all electricity consumption in the country, at a cost of $\$4.5$ billion \cite{Vrbsky10}. The power consumption of data centers and the network infrastructure is predicted to reach $10,300$ TWh/year\footnote{One TWh (Tera Watt Hour) is equal to $10^{12}$ Wh.} in $2030$, based on $2010$ levels of efficiency \cite{Preist10}. These increases are expected in spite of the extraordinary reduction in  energy requirements for computing activities; over the past $30$ years the energy efficiency per transistor on a chip has improved by six orders of magnitude.


The energy costs are passed down to the users of cloud services and differ from one region to another. For example, a medium utilization reserved instance for quadruple extra-large reserved memory EC2 instance requires an upfront payment of $\$2,604$ for a one year term and $\$0.412$ per hour for the US East (N. Virginia) AWS region. The same instance costs $ \$5,632$ upfront and $\$0.724$ per hour for the South America (Sao Paolo) region \cite{Amazon13}.  The energy costs for the two regions differ by about $\$40\%$. The higher energy and networking cost are responsible for the significant price difference in this example.

We have witnessed improvements in the energy efficiency of computing - the number of computation completed per kilowatt-hour of electricity. We have also seen an improvement of data centers energy efficiency. A measure of the energy efficiency of a data center, the so-called PUE (power usage effectiveness), is the ratio of the total energy used to power a data center to the energy used to power computational servers, storage servers, routers, and other IT equipment. The PUE has improved from around $1.93$ in 2003 to $1.63$ in 2005. Recently, it was reported that Goggle's PUE ratio is now as low as 1.15 \cite{Baliga11}.

{\bf Economy of scale.} A public cloud provides services to large user community with diverse applications; the hardware is shared my multiple customers and applications. The users access the public cloud from anywhere in the Internet and only pay for the services they use. A private cloud serves a single organization, typically maintained behind a firewall and accessed through an intranet. A set of diverse applications may run on a private cloud. An organization may purchase its own private, isolated group of servers from public cloud service providers such as Amazon  or Rackspace.

Economy of scale, affects the energy efficiency of data processing. For example, Google reports that the annual energy consumption for an Email service varies significantly depending on the business size and can be 15 times larger for a small one than for large business (Google 2013). Cloud computing can be more energy efficient than on-premise computing for many organizations \cite{Baliga11, NRDC12}. The energy used to transport the data is a significant component of the total energy cost and according to \cite{Baliga11} ''a public cloud could consume three to four times more power than the private cloud due to increased energy consumption in transport.''

The power consumption of servers has increased over time. Table \ref{ServerEnergyConsumption}  \cite{Koomey07} shows the evolution of the average power consumption for volume (Vol) servers - servers with a price less than \$ 25 K, mid-range (Mid) servers - servers with a price between \$25 K and \$499 K, and high-end (High) servers - servers with a price tag larger than \$500 K.

\begin{table*}[!ht]
\begin{center}
\caption{Estimated average power use of volume, mid-range, and high-end servers (in Watts) along the years \cite{Koomey07}.}
\label{ServerEnergyConsumption}
\begin{tabular} {|c|ccccccc|}
\hline
Type   & 2000  & 2001  & 2002  & 2003  & 2004  & 2005  & 2006 \\
\hline
Vol    & 186   & 193   & 200   & 207   & 213   & 219   & 225 \\
Mid    & 424   & 457   & 491   & 524   & 574   & 625   & 675 \\
High   & 5,534 & 5,832 & 6,130 & 6,428 & 6,973 & 7,651 & 8,163 \\
 \hline
\end{tabular}
\end{center}
\end{table*}


{\bf Energy for communication with the cloud.} Cloud computing is only possible because the Internet allows user access to the large data centers. But the Internet itself consumes a fair amount of energy. This amount is likely to increase dramatically,  the hourly Internet traffic will shortly exceed the annual traffic in the year 2000 \cite{Mills13}!!

A recent study \cite{CEET13} warns that ``…access networks, not data centers, are the biggest  threat to the sustainability of cloud services. This is because more people are accessing cloud services via wireless networks. These networks are inherently energy inefficient and a disproportionate contributor to cloud energy consumption .... . cloud services accessed via wireless networks is expected to grow up to $460\%$ between 2012 and 2015, the equivalent of $4.9$ million new cars on the roads….. wireless access networks will be responsible for $90\%$ of that energy.''

The increased energy efficiency of the cloud infrastructure, though significant, had a relatively small impact on the total energy used for cloud-related activities.  In recent years we have seen a dramatic increase in the number of mobile devices which access data stored on the cloud and this leads to a significant increase in the energy used to transfer data to and from the clouds. 

The support for network centric content consumes a very large fraction of the network bandwidth; according to the CISCO VNI forecast in 2009 consumer traffic was responsible for around $80\%$ of the bandwidth used and is expected to grow at a faster rate than business traffic. Data intensity for different activities varies widely \cite{Preist10}: 20 MB/minute for HDTV streaming; 10 MB/minute for Standard TV streaming; 1.3 MB/minute for music streaming, 0.96 MB/minute for Internet radio; 0.35 MB/minute for Internet browsing; and 0.0025 MB/minute for Ebook reading.

The same study reports that if the energy demand for bandwidth is 4 Watts-hour per MB and if the demand for network bandwidth is $3.2$ GB/day/person or $2,570$ EB/year for the entire world population, then the energy required for this activity will be $1,175$ GW.  These estimates do not count very high bandwidth applications that may emerge in the future, such as 3D-TV, personalized immersive entertainment, such as Second Life, or massively multi-player online games. As we have seen in Section 3, the power consumption of the networking infrastructure is significant; as the volumes of data transferred to and from a cloud increase the power consumption for networking will also increase.


{\bf The carbon footprint.} Reduction of the carbon footprint can only be achieved through a comprehensive set of technical efforts. The hardware of the cloud infrastructure has to be refreshed periodically and new and more energy efficient technologies have to be adopted, the resource management software has to pay more attention to energy optimization, the housing and cooling cost have to be reduced, and last, but not least, more energy for powering the cloud infrastructure should come from renewable energy sources.

A comprehensive report released in 2012 \cite{NRDC12} identifies four major factors which affect the carbon emissions of different types of IT activities: (i) The  ratio of the total energy consumption of a center to the fraction of energy used to power the servers and the routers of the center (PUE); (ii) The average server utilization (U) - the lower the less efficient energy efficiency; (iii) The refresh period of the equipment (P) - the time between successive replacements of the equipment with the newer ones; And the ratio (R) of virtualized servers versus non-virtualized ones. For example, for a public cloud assuming an average scenario when the PUE is $1.5$, the average server utilization is $40\%$, the refresh period of the equipment is two years and the ratio of virtualized to non-virtualized servers is eight to one the emission factor measured in kilograms of CO2 equivalent per kilowatt-hour is $0.554$. This factor improves to $0.268$ for a best case scenario, (PUE=1.1, $U=70\%$, P=1 year, R=12/1), but worsens to $0.819$ for a worst case scenario (PUE=2.0, $U=7\%$, P=3 years, R=5/1).



